Counting Hyperelliptic curves on Abelian surfaces with Quasi-modular forms

In this paper we produce a generating function for the number of hyperelliptic curves (up to translation) on a polarized Abelian surfaces using the crepant resolution conjecture and the Yau-Zaslow formula. We present a formula to compute these in terms of MacMahon's generalized sum-of-divisors functions, and prove that they are quasi-modular forms.

==> headers.tex <==
%!TEX root = paper.tex
\usepackage{pb-xy,pb-diagram}
\usepackage{amssymb,amsmath,amsthm}
%\usepackage[pdftex]{graphicx,color}  
\usepackage{graphicx}
%\usepackage{enumitem}
\usepackage{mathrsfs}

\usepackage[all]{xy}
 
 \theoremstyle{plain}
 \newtheorem{theorem}{Theorem}[chapter]
 \newtheorem{proposition}[theorem]{Proposition}
 \newtheorem{lemma}[theorem]{Lemma}
 \newtheorem{corollary}[theorem]{Corollary}
 \newtheorem{conjecture}[theorem]{Conjecture}
 \newtheorem{question}[theorem]{Question}
 \newtheorem*{theorem*}{Theorem}
 \newtheorem*{proposition*}{Proposition}
 \newtheorem*{lemma*}{Lemma}
 \newtheorem*{corollary*}{Corollary}
 \newtheorem*{conjecture*}{Conjecture}
 
 
 %\newcommand{\localdef}{}

%\newenvironment{definition}[1]{\begin{trivlist}\item [\hskip \labelsep {\bfseries Definition \addtocounter{theorem}{1}\thetheorem}]\renewcommand{\localdef}{\index{#1}{\em #1 }}}{\end{trivlist}}

\newenvironment{definition}{\refstepcounter{theorem}\begin{trivlist}\item [\hskip \labelsep {\bfseries Definition \thetheorem}]}{\end{trivlist}}


\theoremstyle{remark}

\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}


\newenvironment{notation}[1][Notation]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

 

 \theoremstyle{plain}

\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\U}{\mathbb{H}}
\newcommand{\F}{\mathbb{F}}
\newcommand{\PP}{\mathbb{P}}

\newcommand{\bk}{{\bf k}}
\newcommand{\zp}{\mathbb{Z}_{\geq 0}}

\newcommand{\setless}[2]{#1\setminus\{#2\}}

\newcommand{\srarrow}{\twoheadrightarrow}
\newcommand{\irarrow}{\rightarrowtail}

\newcommand{\conj}[1]{\overline{#1}}

\newcommand{\factor}[2]{\raisebox{0.1ex}{$#1$}\raisebox{-0.3ex}{/}\raisebox{-0.9ex}{$#2$}}

\newcommand{\tchar}[2]{\genfrac{[}{]}{0pt}{}{#1}{#2}}

%\newcommand{\moda}[2]{\overline{M}_{0;#1}\big([A/\pm1], #2\big)}
%\newcommand{\moda}[2]{\overline{M}\big([A/\pm1]; #1; #2\big)}
\newcommand{\moda}[3][{[A/\pm1]}]{\overline{M}\left(#1; #2; #3\right)}
\newcommand{\modac}[2]{M^\circ\left([A/\pm1]; #1; #2\right)}

\newcounter{Lcount}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% These two are just because I'm lazy and \tilde and \hat
% are nearly impossible to see.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\tilde}{\widetilde}
\renewcommand{\hat}{\widehat}

\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\vdim}{vdim}
\DeclareMathOperator{\map}{Map}
\DeclareMathOperator{\Km}{Km}

